An Examination of Offline-Trained Encoders in Vision-Based Deep Reinforcement Learning for Autonomous Driving

Our research investigates the challenges Deep Reinforcement Learning (DRL) faces in complex, Partially Observable Markov Decision Processes (POMDP) such as autonomous driving (AD), and proposes a solution for vision-based navigation in these environments. Partial observability reduces RL performance significantly, and this can be mitigated by augmenting sensor information and data fusion to reflect a more Markovian environment. However, this necessitates an increasingly complex perception module, whose training via RL is complicated due to inherent limitations. As the neural network architecture becomes more complex, the reward function's effectiveness as an error signal diminishes since the only source of supervision is the reward, which is often noisy, sparse, and delayed. Task-irrelevant elements in images, such as the sky or certain objects, pose additional complexities. Our research adopts an offline-trained encoder to leverage large video datasets through self-supervised learning to learn generalizable representations. Then, we train a head network on top of these representations through DRL to learn to control an ego vehicle in the CARLA AD simulator. This study presents a broad investigation of the impact of different learning schemes for offline-training of encoders on the performance of DRL agents in challenging AD tasks. Furthermore, we show that the features learned by watching BDD100K driving videos can be directly transferred to achieve lane following and collision avoidance in CARLA simulator, in a zero-shot learning fashion. Finally, we explore the impact of various architectural decisions for the RL networks to utilize the transferred representations efficiently. Therefore, in this work, we introduce and validate an optimal way for obtaining suitable representations of the environment, and transferring them to RL networks.

==> Conclusion.tex <==
\section{Conclusion}
Our research supports the central importance of representation learning to the success of RL approaches. Despite similar configurations and comparable capacities of the RL neural networks used, we found significant differences in the performance of the systems. Recent advances in SSL, particularly the use of pre-trained encoders for downstream tasks, find confirmation in our specific application scenario: AD using RL. Here, the performance of the RL agent mirrors the performance observed in other downstream tasks in the work of Feichtenhofer et al. \cite{SSL3DRL}. For example, the performances of MoCo and BYOL were similarly good, while DPC's results from their official work \cite{DPC2019} tested on the same datasets and downstream tasks performed significantly worse. Despite the promising results with SSL, SL remains the most effective approach for training NNs. The often-discussed question of whether RL works on significant complex problems is closely related to the proper representation of the spatiotemporal input data. We have shown that the quality of the policies obtained is closely related to the quality of the underlying representation.

Finally, our results highlight the inherent difficulty of learning representations based on reward-driven loss. It confirms the need to separate these processes and optimize them individually. This finding makes a valuable contribution to further developing effective and efficient RL methods.

\paragraph{Future Work}
As for future work, one straightforward extension of this idea is to use a larger NN as a backbone, such as ResNet50. Also, the AD task will be extended to include the acceleration axis to test the RL agent more effectively. Namely, for successful control of acceleration, features must capture the dynamics of the environment around the ego vehicle.
